Quasar Sightline and Galaxy Evolution (QSAGE) Survey - I. The Galaxy Environment of OVI Absorbers up to z=1.4 around PKS 0232-04

We present the first results from a study of OVI absorption around galaxies at $z<1.44$ using data from a near-infrared grism spectroscopic Hubble Space Telescope Large Program, the Quasar Sightline and Galaxy Evolution (QSAGE) survey. QSAGE is the first grism galaxy survey to focus on the circumgalactic medium at $z\sim1$, providing a blind survey of the galaxy population. Using the first of 12 fields, we provide details of the reduction methods, in particular the handling of the deep grism data which uses multiple position angles to minimise the effects of contamination from overlapping traces. The resulting galaxy sample is H$\alpha$ flux limited ($f({\rm H\alpha}) > 2\times10^{-17}$ erg s$^{-1}$ cm$^{-2}$) at 0.68<z<1.44, corresponding to $\gtrsim0.2-0.8$ M$_\odot$ yr$^{-1}$. We combine the galaxy data with high-resolution STIS and COS spectroscopy of the background quasar to study OVI in the circumgalactic medium. At z>0.68, we find 5 OVI absorption systems along the line of sight with identified galaxies lying at impact parameters of $b\approx100-350$ kpc (proper), whilst we find a further 13 galaxies with no significant associated OVI absorption (i.e. $N({\rm OVI})<10^{13.5-14}$ cm$^{-2}$) in the same impact parameter and redshift range. We find a large scatter in the stellar mass and star-formation rates of the closest galaxies with associated OVI. Whilst one of the OVI absorber systems is found to be associated with a low mass galaxy group at $z\approx1.08$, we infer that the detected OVI absorbers typically lie in the proximity of dark matter halos of masses $10^{11.5} {\rm M_\odot}\lesssim M_{\rm halo}\lesssim10^{12} {\rm M_\odot}$.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
